Specularity Factorization for Low-Light Enhancement

We present a new additive image factorization technique that treats images to be composed of multiple latent specular components which can be simply estimated recursively by modulating the sparsity during decomposition. Our model-driven {\em RSFNet} estimates these factors by unrolling the optimization into network layers requiring only a few scalars to be learned. The resultant factors are interpretable by design and can be fused for different image enhancement tasks via a network or combined directly by the user in a controllable fashion. Based on RSFNet, we detail a zero-reference Low Light Enhancement (LLE) application trained without paired or unpaired supervision. Our system improves the state-of-the-art performance on standard benchmarks and achieves better generalization on multiple other datasets. We also integrate our factors with other task specific fusion networks for applications like deraining, deblurring and dehazing with negligible overhead thereby highlighting the multi-domain and multi-task generalizability of our proposed RSFNet. The code and data is released for reproducibility on the project homepage.

==> results.tex <==
\begin{figure*}
\begin{tabular}{ccc}
    \includegraphics[width=0.33\linewidth, height=4cm]{DICM_01.jpg} &
     \includegraphics[width=0.33\linewidth, height=4cm]{DICM_59.jpg} &
     \includegraphics[width=0.33\linewidth, height=4cm]{DICM_16.jpg} \\
     
    \includegraphics[width=0.33\linewidth, height=3cm]{DICM_15.jpg} &
     \includegraphics[width=0.33\linewidth, height=3cm]{DICM_17.jpg} &
     \includegraphics[width=0.33\linewidth, height=3cm]{DICM_33.jpg} \\
     
    \includegraphics[width=0.33\linewidth, height=3cm]{DICM_28.jpg} &
     \includegraphics[width=0.33\linewidth, height=3cm]{DICM_37.jpg} &
     \includegraphics[width=0.33\linewidth, height=3cm]{DICM_41.jpg} \\
     
    \includegraphics[width=0.33\linewidth, height=3cm]{8.jpg} &
     \includegraphics[width=0.33\linewidth, height=3cm]{10.jpg} &
     \includegraphics[width=0.33\linewidth, height=3cm]{1.jpg} \\
     
    \includegraphics[width=0.33\linewidth, height=3cm]{2.jpg} &
     \includegraphics[width=0.33\linewidth, height=3cm]{Candle.jpg} &
     \includegraphics[width=0.33\linewidth, height=3cm]{BelgiumHouse.jpg} \\

     \includegraphics[width=0.33\linewidth, height=3cm]{House.jpg} &
     \includegraphics[width=0.33\linewidth, height=3cm]{Kluki.jpg} &
     \includegraphics[width=0.33\linewidth, height=3cm]{Office.jpg} \\
     
\end{tabular}
\caption{LLE Results: We show several input (red box) and our enhanced output (green box) pairs, generated using our RSFNet. }
\label{fig:LLEres_1}
\end{figure*}
% -----------------------------------------------------------------
\begin{figure*}
\begin{tabular}{ccc}
    \includegraphics[width=0.33\linewidth, height=4cm]{r072649fdt.jpg} &
     \includegraphics[width=0.33\linewidth, height=4cm]{r077507cat.jpg} &
     \includegraphics[width=0.33\linewidth, height=4cm]{r097088c1t.jpg} \\
     
    \includegraphics[width=0.33\linewidth, height=3cm]{r107730b5t.jpg} &
     \includegraphics[width=0.33\linewidth, height=3cm]{r125034a9t.jpg} &
     \includegraphics[width=0.33\linewidth, height=3cm]{r145221d9t.jpg} \\
     
    \includegraphics[width=0.33\linewidth, height=3cm]{r146771d7t.jpg} &
     \includegraphics[width=0.33\linewidth, height=3cm]{r0708431at.jpg} &
     \includegraphics[width=0.33\linewidth, height=3cm]{r00869422t.jpg} \\
     
    \includegraphics[width=0.33\linewidth, height=3cm]{r01559391t.jpg} &
     \includegraphics[width=0.33\linewidth, height=3cm]{r1904147dt.jpg} &
     \includegraphics[width=0.33\linewidth, height=3cm]{r02354285t.jpg} \\
     
    \includegraphics[width=0.33\linewidth, height=3cm]{r02508493t.jpg} &
     \includegraphics[width=0.33\linewidth, height=3cm]{r05243256t.jpg} &
     \includegraphics[width=0.33\linewidth, height=3cm]{r01559391t.jpg} \\

     \includegraphics[width=0.33\linewidth, height=3cm]{r14289905t.jpg} &
     \includegraphics[width=0.33\linewidth, height=3cm]{r17217693t.jpg} &
     \includegraphics[width=0.33\linewidth, height=3cm]{r141665bdt.jpg} \\
     
\end{tabular}
\caption{LLE Results: We show several input (red box) and our enhanced output (green box) pairs, generated using our RSFNet. }
\label{fig:LLEres_2}
\end{figure*}
% -----------------------------------------------------------------
\begin{figure*}
        \includegraphics[width=\linewidth, height=3cm]{22.jpg} \\
        \includegraphics[width=\linewidth, height=3cm]{111.jpg} \\
        \includegraphics[width=\linewidth, height=3cm]{493.jpg} \\
        \includegraphics[width=\linewidth, height=3cm]{547.jpg} \\
        \includegraphics[width=\linewidth, height=3cm]{669.jpg} \\
        \includegraphics[width=\linewidth, height=3cm]{00720.jpg} \\
        \includegraphics[width=\linewidth, height=3cm]{00737.jpg} \\
\caption{Factors Visualization: For a given scene represented with the ground truth image  (green box), we show five factors (blue boxes) that we obtain using our proposed factorization. Note that the factorization is done on the corresponding LLE image (not shown) and images here are rescaled for visualization.}
\label{fig:facViz_1}
\end{figure*}

\begin{figure*}
        \includegraphics[width=\linewidth, height=3cm]{748.jpg} \\
        \includegraphics[width=\linewidth, height=3cm]{00749.jpg} \\
        \includegraphics[width=\linewidth, height=3cm]{00757.jpg} \\
        \includegraphics[width=\linewidth, height=3cm]{00774.jpg} \\
        \includegraphics[width=\linewidth, height=3cm]{00776.jpg} \\
        \includegraphics[width=\linewidth, height=3cm]{00784.jpg} \\
        \includegraphics[width=\linewidth, height=3cm]{00787.jpg} \\
\caption{Factors Visualization: For a given scene represented with the ground truth image  (green box), we show five factors (blue boxes) that we obtain using our proposed factorization. Note that the factorization is done on the corresponding LLE image (not shown) and images here are rescaled for visualization.}
\label{fig:facViz_2}
\end{figure*}
% -----------------------------------------------------------------
\begin{figure*}
    \includegraphics[width=\linewidth, height=3cm]{P1020044.jpg} \\
    \includegraphics[width=\linewidth, height=3cm]{night_25.jpg} \\
    \includegraphics[width=\linewidth, height=3cm]{cloudy_20.jpg} \\
    \includegraphics[width=\linewidth, height=3cm]{Daybreak-Nightfall_8.jpg} \\
    \includegraphics[width=\linewidth, height=3cm]{cloudy_6.jpg} \\
    \includegraphics[width=\linewidth, height=3cm]{10.jpg} \\
    \includegraphics[width=\linewidth, height=3cm]{28.jpg} \\
    \caption{Qualitative Comparison: We show results for a given input image (left, red box) from various methods. Left-to-right: Ours (green box), zeroDCE, zeroDCE++, RUAS, SCI and PSENet. zeroDCE and zeroDCE++ ($3^{rd}$, $4^{th}$ columns) have colors and contrast with unnatural look. RUAS and SCI ($5^{th}$, $6^{th}$ columns) are not able to handle overexposed regions. PSENet (right) on the other hand over saturates color values. Our results ($1^{st}$ column) overall present a naturally enhanced version of the input. }
    \label{fig:qual_compare}
\end{figure*}
% % -----------------------------------------------------------------
% \begin{figure*}
% \begin{tabular}{ccc}
% \includegraphics[width=0.3\linewidth,height=3cm]{assets/Supp/Control/blackCloud/1.jpg} &
% \includegraphics[width=0.3\linewidth,height=3cm]{assets/Supp/Control/blackCloud/2.jpg} &
% \includegraphics[width=0.3\linewidth,height=3cm]{assets/Supp/Control/blackCloud/3.jpg} \\
% \includegraphics[width=0.3\linewidth,height=3cm]{assets/Supp/Control/blackCloud/4.jpg} &
% \includegraphics[width=0.3\linewidth,height=3cm]{assets/Supp/Control/blackCloud/5.jpg} &
% \includegraphics[width=0.3\linewidth,height=3cm]{assets/Supp/Control/blackCloud/6.jpg} \\
% \end{tabular}
%     \caption{User edited results: Here we show multiple images \textit{with dark clouds} which can be generated by manipulating the specular factors with various image processing operations before fusion.}
%     \label{fig:control_1}
% \end{figure*}
% \begin{figure*}
% \begin{tabular}{ccc}
% \includegraphics[width=0.3\linewidth,height=3cm]{assets/Supp/Control/colorEnahnce/1.jpg} &
% \includegraphics[width=0.3\linewidth,height=3cm]{assets/Supp/Control/colorEnahnce/2.jpg} &
% \includegraphics[width=0.3\linewidth,height=3cm]{assets/Supp/Control/colorEnahnce/3.jpg} \\
% \includegraphics[width=0.3\linewidth,height=3cm]{assets/Supp/Control/colorEnahnce/4.jpg} &
% \includegraphics[width=0.3\linewidth,height=3cm]{assets/Supp/Control/colorEnahnce/5.jpg} &
% \includegraphics[width=0.3\linewidth,height=3cm]{assets/Supp/Control/colorEnahnce/6.jpg} \\
% \end{tabular}
%     \caption{User edited results: Here we show multiple images \textit{enhanced colors} which can be generated by manipulating the specular factors with various image processing operations before fusion.}
%     \label{fig:control_2}
% \end{figure*}
% \begin{figure*}
% \begin{tabular}{ccc}
% \includegraphics[width=0.3\linewidth,height=3cm]{assets/Supp/Control/blackSky/1.jpg} &
% \includegraphics[width=0.3\linewidth,height=3cm]{assets/Supp/Control/blackSky/2.jpg} &
% \includegraphics[width=0.3\linewidth,height=3cm]{assets/Supp/Control/blackSky/3.jpg} \\
% \includegraphics[width=0.3\linewidth,height=3cm]{assets/Supp/Control/blackSky/4.jpg} &
% \includegraphics[width=0.3\linewidth,height=3cm]{assets/Supp/Control/blackSky/5.jpg} &
% \includegraphics[width=0.3\linewidth,height=3cm]{assets/Supp/Control/blackSky/6.jpg} \\
% \end{tabular}
%     \caption{User edited results: Here we show multiple images \textit{dark sky} which can be generated by manipulating the specular factors with various image processing operations before fusion.}assets/Supp/Compare/
%     \label{fig:control_3}
% \end{figure*}

